FedHyper: A Universal and Robust Learning Rate Scheduler for Federated Learning with Hypergradient Descent

The theoretical landscape of federated learning (FL) undergoes rapid evolution, but its practical application encounters a series of intricate challenges, and hyperparameter optimization is one of these critical challenges. Amongst the diverse adjustments in hyperparameters, the adaptation of the learning rate emerges as a crucial component, holding the promise of significantly enhancing the efficacy of FL systems. In response to this critical need, this paper presents FedHyper, a novel hypergradient-based learning rate adaptation algorithm specifically designed for FL. FedHyper serves as a universal learning rate scheduler that can adapt both global and local rates as the training progresses. In addition, FedHyper not only showcases unparalleled robustness to a spectrum of initial learning rate configurations but also significantly alleviates the necessity for laborious empirical learning rate adjustments. We provide a comprehensive theoretical analysis of FedHyper's convergence rate and conduct extensive experiments on vision and language benchmark datasets. The results demonstrate that FEDHYPER consistently converges 1.1-3x faster than FedAvg and the competing baselines while achieving superior final accuracy. Moreover, FedHyper catalyzes a remarkable surge in accuracy, augmenting it by up to 15% compared to FedAvg under suboptimal initial learning rate settings.

==> 3_method_x.tex <==
\section{Proposed Method: FedHyper}\label{sec:method}
%\JW{Need to firstly introduce what is a leanring rate and what is a good learning rate schedule.}
\textbf{Gradient Descent and Learning Rate.} Gradient descent~\citep{ruder2016overview} is the most widely used optimization method in machine learning. During the iterative steps of gradient descent, the new model parameter $W^{t+1}$ in $(t+1)$th step is determined by the previous parameter $W^t$, the model gradient $\nabla F(W^t)$ with respect to the loss function, and the learning rate $\eta^t$:
\begin{equation}
\label{eq:gdgd}
W^{t+1} = W^t - \eta^t \cdot \nabla F(W^t).
\end{equation}

Thus, the learning rate acts as a hyperparameter that determines the step size of updating the model~\citep{murphy2012machine}. 
%In FL, it refers to the step sizes in the server aggregation process, i.e., the global learning rate, and the local SGD process, i.e., the local learning rate. 
Although the learning rate is preset, it also can be adjusted during the training process by a scheduler~\citep{wen2021convolutional} in order to make the training more efficient. It is a consensus that in the early training stages, a larger learning rate is often needed to rapidly bring the model parameters closer to the global optimum. In the later stages, a smaller learning rate is required for fine-tuning the model to achieve minimal loss. Therefore, an ideal learning rate scheduler should start with a relatively high learning rate in the initial training phase and gradually reduce it as training progresses. In order to construct a mathematical model for this ideal scheduler, we assert that the change in the learning rate is continuous in the model training process. Therefore, the optimal updating strategy for the learning rate can be defined as a function related to the previous step's learning rate, which is:
\begin{equation}
\label{eq:lr}
\eta^t = f(\eta^{t-1}),
\end{equation}
where $\eta^t$ and $\eta^{t-1}$ are the learning rates in $t$th and $(t-1)$th training steps respectively. $f(\eta^{t-1})$ serves as an ideal predictive function for the new learning rate $\eta^t$, given the knowledge of the last learning rate $\eta^{t-1}$. This function can update the learning rate to its optimal value in $t$th step. However, we cannot get the ideal function in real model training situations. Hence, what we can do is to use a substitute pre-defined function to approximate $f(\eta^{t-1})$.
\JW{$L$ is often used to refer to the loss function. Please change to $\alpha, \beta$ or $\gamma$.}

\textbf{Hypergradient Descent.} Hypergradient descent is designed for this approximation during the practical process. The key idea of it is to approximate $f(\eta^{t-1})$ as a gradient descent function. It calculates the derivation of the learning rate $\eta^t$ with respect to the loss during the model training and updates $\eta^t$ from $\eta^{t-1}$ by the gradient direction that can minimize the training loss. Specifically, it first calculates the derivation of $\eta^t$ from the gradient descent process in Eq. \ref{eq:gdgd}:
\begin{equation}
\label{eq:gderi}
\begin{split}
\frac{\partial F(W^{t+1})}{\partial \eta^t} &= \nabla F(W^{t+1}) \cdot \frac{\partial (W^{t} - \eta^t \nabla F(W^{t}))}{\partial \eta^t} \\
&=-\nabla F(W^{t+1})\cdot\nabla F(W^{t}).
\end{split}
\end{equation}

However, $\nabla F(W^{t+1})$ is not available in $t$th step, so we approximate $\frac{\partial F(W^{t+1})}{\partial \eta^t}$ by $\frac{\partial F(W^{t})}{\partial \eta^{t-1}}$, and then gets the following update rule for $\eta^t$:
\begin{equation}
\label{eq:alphaa}
\widetilde{\frac{\partial F(W^{t+1})}{\partial \eta^t}}= \frac{\partial F(W^{t})}{\partial \eta^{t-1}} = -\nabla F(W^{t})\cdot\nabla F(W^{t-1}).
\end{equation}

Therefore, in order to minimize $F(W^{t+1})$, we update $\eta^t$ by hypergradient descent on $\eta^{t-1}$:
\begin{equation}
\label{eq:alpha}
\begin{split}
\eta^t &= \eta^{t-1} - \widetilde{\frac{\partial F(W^{t+1})}{\partial \eta^t}}\\
&= \eta^{t-1} + \nabla F(W^{t})\cdot\nabla F(W^{t-1}).
\end{split}
\end{equation}

This strategy suggests that the learning rate at the $t$th step, $\eta^t$, should be the sum of the previous step's learning rate, $\eta^{t-1}$, and the product of the model gradients at the $t$th and $(t-1)$th steps. Specifically, if the dot product $\nabla F(W^{t})\cdot\nabla F(W^{t-1})$ is positive, indicating that the global gradients from the last two steps are in similar directions, the learning rate will increase.
Conversely, a negative value suggests divergent gradient directions, leading to a decrease in the learning rate. This adaptive approach tailors the learning rate based on training dynamics.
To illustrate this adaptability,  we present a rudimentary convex optimization task, $\arg\min_x x^2$, as a demonstrative example, depicted in Figure \ref{fig:G}. As Figure \ref{fig:G1} shows, the model parameters in $t-1$th and $t$th steps, namely $W^{t-1}$ and $W^{t}$, are far from the optimal parameter $W^{opt}$, requiring a larger learning rate for expedited training. 
According to the hypergradient descent in Eq. \ref{eq:alpha}, the hypergradient of $\eta^t$ (represented as $\Delta^t\cdot\Delta^{t-1}$) is positive, given their aligned gradient directions. Therefore, $\eta^t$ is larger than $\eta^{t-1}$, facilitating a faster convergence towards $W_{opt}$.

In Figure \ref{fig:G2}, $W^{t-1}$ is close to $W^{opt}$. 
However, the magnitude of the model update from the $(t-1)$th step, represented by $\Delta^{t-1}\cdot \eta^{t-1}$, is so substantial that it overshoots $W^{opt}$, landing on its opposite side. 
In this scenario, a reduced learning rate is desirable to guide the parameter gently towards $W^{opt}$.
Given that the hypergradient of $\eta^t$ is negative, i.e., owing to the opposing directions of $\Delta^{t}$ and $\Delta^{t-1}$, the learning rate $\eta^t$ will be decreased relative to $\eta^{t-1}$. Consequently, the subsequent update for $W^{t+1}$ will utilize this more appropriate, reduced learning rate, ensuring a closer approximation to $W^{opt}$.

\begin{figure}[]
\centering
\subfigure[Performance of FedHyper-G]{\centering
\includegraphics[width=0.4\textwidth]{G1.png}\label{fig:G1}}
\subfigure[Performance of FedHyper-G]{\centering
\includegraphics[width=0.4\textwidth]{G2.png}\label{fig:G2}}
\caption{Two situations in hypergradient descent. Hypergradient descent can adjust the learning rate according to the training progress.}
\label{fig:G}
\end{figure} 

Hypergradient descent works well in centralized ML,
%and outperforms baselines such as SGD~\citep{bottou2010large} and Adam~\citep{kingma2014adam}. 
%\JW{I think this statement could be controversial. Apparently, Adam is still the default optimizer for most researchers and practitioners. Do we really need to mention this?}
but it faces challenges in FL due to the collaborative nature of FL across multiple devices and the data heterogeneity. Specifically, for the learning rate schedulers on the server, $\nabla F(W)$ is not available because the server does not possess its own training dataset to perform gradient calculations. So we cannot directly apply Eq. \ref{eq:alpha} to the global scheduler. For the client scheduler, simply applying a hypergradient descent to clients may lead to excessive local learning rates for some clients with easy-to-train datasets. If among them, there are local updates that exhibit significant deviations from the overall task, it will hinder the global model convergence, especially in non-iid setting~\citep{wang2020tackling}.

To address these challenges, we develop {\n}, a scheduler based on hypergradient descent specifically designed for FL. {\n} comprises a global scheduler \textsc{FedHyper-G}, a server-side local scheduler \textsc{FedHyper-SL} and a client-side local scheduler \textsc{FedHyper-SC}. \textsc{FedHyper-G} and \textsc{FedHyper-SL} are based on the hypergradient of the global learning rate $\alpha$ while \textsc{FedHyper-SC} is based on hypergradient of the local learning rate $\beta$.

\textbf{Global Scheduler: FedHyper-G.} 
Adjusting learning rates on the server is efficient because the global aggregation process consumes very little time, compared with multi-step local SGD. Therefore, we provide \textsc{FedHyper-G} to adjust the global learning rate $\alpha$ based on the hypergradient descent in the global model update process. According to Eq. \ref{eq:alpha}, the new global learning rate in $t$th round, i.e., $\alpha^t$ should be computed by the last global learning rate $\alpha^{t-1}$ and global gradients in the last two rounds. However, in accordance with the strategy of \textsc{FedAvg}, the global model is updated by the aggregation of local model updates rather than gradients:
\begin{equation}
\label{eq:avgup}
\begin{split}
W^{t+1} &= W^t - \alpha^t \cdot \Sigma P_m \Delta_m^t \\
&= W^t - \alpha \cdot \Delta^t 
\end{split}
\end{equation}
where $\Delta_m^t$ is the local model update in $t$th round and $P_m$ is the corresponding weight for aggregation. $\Delta^t$ is the global model update averaged by local updates. Therefore, in \textsc{FedHyper-G}, we treat $\Delta^t$ as the pseudo global gradient and express the Eq. \ref{eq:alpha} in a form adapted for global scheduler:
\begin{equation}
\label{eq:alphafl}
\alpha^t = \alpha^{t-1} + \Delta^t\cdot\Delta^{t-1}
\end{equation}

In addition, to ensure convergence and prevent gradient exploration, we clip $\alpha^t$ by a preset bound value $\gamma_\alpha$ in each round:
\begin{equation}
\label{eq:gamma}
\alpha_t = \min \{ \max \{ \alpha_t, \frac{1}{\gamma_{\alpha}} \}, \gamma_{\alpha} \}
\end{equation}
%\JW{Need to mention that $\gamma$ is easy to tune in practice. For example, whether a simple value works well for all datasets?}

Through experiments, we have found that setting $\gamma_\alpha$ to 3 results in stable performance for various tasks and configurations in \textsc{FedHyper-G}. Therefore, we generally do not need to further adjust $\gamma_\alpha$.

\textbf{Server-side Local Scheduler: FedHyper-SL.} The server-side local scheduler adopts the same hypergradient as the global scheduler. It adjusts all the local learning rates from selected clients synchronously. The local learning rates are also clipped by a preset bound value $\gamma_\beta$:
\begin{equation}
\label{eq:sls}
\begin{split}
\beta_m^t &= \beta_m^{t-1} + \Delta^t\cdot\Delta^{t-1}, \forall {m} \in \{ 0,1, ..., M \} \\
\beta_m^t &= \min \{ \max \{ \beta_t, \frac{1}{\gamma_{\beta}} \}, \gamma_{\beta} \}
\end{split}
\end{equation}

The updated local learning rates $\beta_m^t$ are sent to clients \emph{after} $t$th round. They will be used by clients in the local updates in the $t+1$th round. Like \textsc{FedHyper-G}, we have experimentally set the value for $\gamma_\beta$ to 10. This bound will also be used for \textsc{FedHyper-CL} mentioned in the following text.

\textbf{Client-side Local Scheduler: FedHyper-CL.}
The global and server-side local schedulers are efficient. However, some FL trainers might expect to use a more fine-grained scheduler to get more performance improvement. To make {\n} also universal for these users, we provide the client-side local scheduler, i.e., \textsc{FedHyper-CL} that adjusts the local learning rate $\beta$ on the clients. \textsc{FedHyper-CL} outperforms \textsc{FedHyper-G} and \textsc{FedHyper-SL} in convergence speed and accuracy because the clients perform more fine-grained adjustment in every local batch, while the server only performs it between communication rounds. With hypergradient descent in Eq. \ref{eq:alpha}, the local learning rate in $k$th local epoch on client $m$ can be updated by:
\begin{equation}
\label{eq:betafl}
\begin{split}
\beta_m^{t,k} &= \beta_m^{t,k-1} + g_m(W_m^{t,k})\cdot g_m(W_m^{t,k-1}) \\
\end{split}
\end{equation}

The $g_m(W_m^{t,k})$ and $g_m(W_m^{t,k-1})$ are the local gradients computed on the adjacent mini-batches. $\beta_m^{t,k}$ is the local learning rate on the $m$th client in $t$th round and $k$th local epch. This local learning rate update strategy tends to minimize local loss $F_m()$ on the local batches. Nevertheless, as mentioned earlier, directly applying hypergradient descent to the local training process will lead to an imbalance in learning rates between clients, which may lead to convergence difficulty.

To solve this problem, inspired by our global scheduler, we aim to introduce global model updates to restrict the local learning rate optimization. Specifically, we add another item $\frac{1}{K} \cdot g_m(W_m^{t,k})\cdot\Delta^{t-1}$ to the local learning rate update, where $\Delta^{t-1}$ is the global model update in the last round and $K$ is the number of local SGD steps:
\begin{equation}
\label{eq:local}
\beta_m^{t,k} =\beta_m^{t,k-1} + g_m(W_m^{t,k})\cdot g_m(W_m^{t,k-1}) + \frac{1}{K} \cdot g_m(W_m^{t,k})\cdot\Delta^{t-1}
\end{equation}

Similarly, $\nabla F_m^\xi(W_m^{t,k})\cdot\Delta^{t-1}$ is a positive number when $\nabla F_m^\xi(W_m^{t,k})$ and $\Delta^{t-1}$ have similar direction, otherwise it is negative. $\frac {1}{K}$ is the coefficient that can adjust $\nabla F_m^\xi(W_m^{t,k})\cdot\Delta^{t-1}$ to be within the same scale as $g_m(W_m^{t,k})\cdot g_m(W_m^{t,k-1})$, since $\Delta^{t-1}$ is the aggregation of $K$ SGD steps. We use This item tends to increase $\beta_m^{t,k}$ when the local model update has a similar direction with the global model update and decrease it when they exhibit significant discrepancies. It can prevent some clients from obtaining excessively high learning rates that could potentially impact global convergence.

This learning rate update rule in Eq.~\ref{eq:local} is more complicated than that in the global update rule. Here we define $X = g_m(W_m^{t,k})\cdot g_m(W_m^{t,k-1}); Y = \frac{1}{K} \cdot g_m(W^{t,k})\cdot\Delta^{t-1}$. The local learning rate in the following four situations will: (1) $X>0; Y>0$ as in Figure~\ref{fig:L1}, increase; (2) $X<0; Y<0$ as in Figure~\ref{fig:L2}, decrease; (3) $X>0; Y<0$ as in Figure~\ref{fig:L3}, increase if $|X|>|Y|$, otherwise decrease; (4) $X<0; Y>0$ as in Figure~\ref{fig:L4}, increase if $|X|<|Y|$, otherwise decrease.

\begin{figure}[]
\centering
\subfigure[$X>0; Y>0$]{\centering
\includegraphics[width=0.23\textwidth]{L1.png}\label{fig:L1}}
\subfigure[$X<0; Y<0$]{\centering
\includegraphics[width=0.23\textwidth]{L2.png}\label{fig:L2}}
\subfigure[$X>0; Y<0$]{\centering
\includegraphics[width=0.23\textwidth]{L3.png}\label{fig:L3}}
\subfigure[$X<0; Y>0$]{\centering
\includegraphics[width=0.23\textwidth]{L4.png}\label{fig:L4}}
\caption{Four situations in client-side local learning rate scheduling.}
\label{fig:local}
\end{figure} 

This client-side local scheduler takes both the global and local training situations into account and adopts global model updates to guide the local learning rate optimization. It enables faster convergence of the local model while preventing excessive client uploads that adversely affect the global model convergence. The full algorithm of the \textsc{FedHyper} schedulers is obtained in Appendix \ref{appen:algor}.


==> 3_preliminary.tex <==
\section{FedAvg and Adaptive Learning Rate}
\label{avg_alr}
%Show limitation of existing works (toy example)

\textbf{Global and Local Update Rule of FedAvg.} In a \textsc{FedAvg} based FL framework with $M$ clients, the $m$th client first performs $K$ steps of local SGD with its local learning rate and computes the local model update $\Delta_m^t$:
\JW{Should be $K$ steps instead of $K$ epochs.}
\begin{equation}
\label{eq:avglo}
\begin{split}
W_m^{t, k+1} &= W_m^{t, k} - \beta_m^{t,k} \cdot g_m(W_m^{t, k}) \\
\Delta_m^t &= W_m^{t, K} - W^t
\end{split}
\end{equation}
where $W_m^{t,k}$ is the model parameters of the $m$th client in the $k$th local epoch in the $t$th communication round, and the initial model parameter sent to clients is $W^t$. $g_m$ represents the stochastic gradient over a mini-batch of client $m$'s local dataset. $\beta_m^{t,k}$ is the local learning rate in the $k$th local epoch.
Then, the global model update rule with $t$th round global learning rate $\alpha^t$ is:
\begin{equation}
\label{eq:avgup}
\begin{split}
W^{t+1} &= W^t - \alpha^t \cdot \Sigma P_m \Delta_m^t \\
&= W^t - \alpha \cdot \Delta^t 
\end{split}
\end{equation}
where $W^t$ denotes the global model parameter and $\Delta^{t}$ is the global model update in $t$th round. $\Delta^{t}$ is averaged by local model updates $\Delta_m^{t}$ with weights $P_m$. 

\textbf{Two Situations in FedAvg.} To demonstrate how the magnitudes of learning rates exert varying effects during the FL training, we visualize a simple convex optimization $\arg\min_x x^2$ in \textsc{FedAvg} with 2 clients in Figure \ref{fig:avg}. The black curve denotes the global optimization objective. It is averaged by the two clients' optimization objectives, which are visualized as blue and red lines. The x-axis of this graph represents the model parameter $W$ in FL, and the y-axis represents the value of the loss $f(W)$. $W^{opt}$ is the optimal global model parameter with the lowest loss.

In the $t$th round, the server sends the global model parameter $W^t$ to two clients. The clients perform local SGD on $W^t$ based on their loss functions and then compute the local model updates $\Delta_0^t$ and $\Delta_1^t$. The server computes $\Delta^t$ by averaging $\Delta_0^t$ and $\Delta_1^t$ to update global model and get $W^{t+1}$. Figure \ref{fig:avg} shows two situations of \textsc{FedAvg}. Figure \ref{fig:avg} (1) is a situation when $W^t$ is far away from the optimal parameter $W_{opt}$. In this case, the clients' model updates $\Delta_0^t$ and $\Delta_1^t$ tend to share the same direction. Therefore, the averaged $\Delta^{t}$ will also have the same direction. Differently, when $W^t$ is close to $W_{opt}$, the local model updates might become diverse, as shown in Figure \ref{fig:avg} (2) where $\Delta_0^t$ and $\Delta_1^t$ have different directions. Therefore, $\Delta^t$ has the same direction as the larger local update.

\begin{wrapfigure}{r}{9.5cm}
\centering
\begin{minipage}[t]{3.0in}
\centering
\includegraphics[trim=0mm 0mm 0mm 0mm,clip,width=2.4in]{toy.png}\\
%\centerline{\footnotesize}
\end{minipage}
\hspace{0cm}
\begin{minipage}[t]{1.8in}
\centering
\includegraphics[trim=0mm 0mm 0mm 0mm, clip,width=1.9in]{far.png}\\
\centerline{\footnotesize (1) Far from Optimum}
\end{minipage}
\hspace{0cm}
\begin{minipage}[t]{1.8in}
\centering
\includegraphics[trim=0mm 0mm 0mm 0mm, clip,width=1.9in]{near.png}\\
\centerline{\footnotesize (2) Close to Optimum}
\end{minipage}
\hspace{0cm}
\begin{minipage}[t]{1.8in}
\centering
\includegraphics[trim=0mm 0mm 0mm 0mm, clip,width=1.93in]{big.png}\\
\centerline{\footnotesize (3) Large Learning Rate}
\end{minipage}
\hspace{0cm}
\begin{minipage}[t]{1.8in}
\centering
\includegraphics[trim=0mm 0mm 0mm 0mm, clip,width=1.93in]{small.png}\\
\centerline{\footnotesize (4) Small Learning Rate}
\end{minipage}
\caption{Two situations in FedAvg.}
\label{fig:avg}
\end{wrapfigure}

\textsc{FedAvg} is capable of accurately computing the direction of $\Delta^{t}$. However, when the global learning rate remains unchanged, it is subject to a trade-off between convergence speed and model accuracy. In situations when the model is far from convergence but uses a small learning rate, such as $\alpha^y$ in Figure \ref{fig:avg} (3), \textsc{FedAvg} may spend a lot of time to reach the optimal point $W_{opt}$. Conversely, using a large learning rate may lead to convergence difficulty when the model is already close to the optimal point like $\alpha^x$ in Figure \ref{fig:avg} (4). Given that the model in FL training typically experiences being far from optimum during the initial rounds, and close to optimum when it approaches convergence, a fixed learning rate is unable to offer good performance.

%Therefore, due to the observation above, an ideal learning rate optimization approach can increase the learning rate when the model is far from convergence, and decrease it when approaching convergence, in order to both speed up training and reach the best performance. In short, the learning rate should be adapted according to the exact training situation.
 \textbf{Learning rate optimization.} Based on the observations mentioned above, an ideal learning rate scheduler should increase the learning rate when the FL model is far from convergence and decrease it when the model approaches convergence. This strategy aims to improve training speed while simultaneously achieving the best accuracy. In summary, the learning rate should be adjusted in response to the specific training situation encountered during FL.

The state-of-the-art learning rate optimization method, \textsc{FedExp}~\citep{jhunjhunwala2023fedexp}, focuses on optimizing the global learning rate. It uses the global model update $\Delta^{t}$ and the local model updates $\Delta_m^t$ to compute the new global learning rate in $t$th round. Then, it selects the maximum value between the computed result and 1 as $\alpha^t$:
\begin{equation}
\label{eq:fedexp}
\alpha^t = \max \left\{1, \frac{\sum_{m=1}^M\|\Delta_m^t\|^2}{2M(\|\Delta^t\|^2 + \epsilon)} \right\}
\end{equation}

\textsc{FedExp} has shown better performance than other global optimization algorithms such as \textsc{FedAdam}, \textsc{FedAdagrad}~\citep{reddi2020adaptive}, and \textsc{SCAFFOLD}~\citep{karimireddy2020scaffold}. However, there are certain limitations associated with it. Firstly, \textsc{FedExp} maintains a global learning rate that is always greater than or equal to 1, which affects the convergence in some tasks suitable for a small global learning rate. Secondly, according to Equation \ref{eq:fedexp}, \textsc{FedExp} suggests using a larger global learning rate when the diversity of local updates increases. This conflicts with the intuition derived from our toy examples presented in Figure \ref{fig:avg}. The situation in Figure \ref{fig:avg} (1) exhibits a lower local gradient diversity, but needs a larger global learning rate, while Figure \ref{fig:avg} (2) has a higher gradient diversity but needs a lower global learning rate. These issues raise concerns that the intuition underlying \textsc{FedExp} may not be effective across different tasks. 

%Therefore, we select to use the gradient of learning rates to guide the optimization. Gradient information can adjust the learning rates according to the actual training situation. Besides, it can also help the optimization of both global and local learning rates, which eliminates the trouble of designing optimization algorithms for different kinds of learning rates.

As a result, we propose using the hypergradient of learning rate realizing its potential to adjust the learning rates in response to the actual training situations. This allows for the rapid adjustment of the learning rate and minimizes the impact of the suboptimal initial learning rate on the training process. Furthermore, compared to algorithms like \textsc{FedExp} that only apply to the global learning rate, our approach can be applied to both global and local learning rates, offering greater versatility.


==> 4_method.tex <==
\section{Our Method: FedHyper}
\label{ours}
In this section, we will first present the derivation process of our global scheduler based on the server gradient information, i.e., \textsc{FedHyper-G}. We then use this optimizer as an inspiration to derive our server-side local scheduler, i.e., \textsc{FedHyper-SL}, and client-side local scheduler, i.e., \textsc{FedHyper-CL}.
\JW{$\textsc{FedHyper-G}$ looks wired. How about \textsc{FedHyper-G}?}

\subsection{Scheduler with $\alpha$ Hypergradient Descent}\label{sub:go}

Adjusting learning rates on the server is efficient because the global aggregation process consumes very little time, compared with multi-epoch local SGD. Therefore, we provide \textsc{FedHyper-G} to adjust the global learning rate $\alpha$ on the server, and \textsc{FedHyper-SL} that adjust the local learning rate $\beta$ on the server.

\textbf{Global scheduler: FedHyper-G.} Our global scheduler adjusts the global learning rate $\alpha$ based on the hypergradient descent in the global model update process.
As shown in Section \ref{avg_alr} and Equation \ref{eq:avgup}, the prospective new model parameter $W^{t+1}$ in $t$th round is computed by $W^t$ and the product of $\alpha^t$ and the global model update $\Delta^t$. 
Here we treat $\Delta^t$ as the pseudo-gradient $\nabla F(W^t)$ of the global model on the overall dataset, from which we can obtain the following equation:
\begin{equation}
\label{eq:ggra}
W^{t+1} = W^t - \alpha^t \cdot \nabla F(W^t)
\end{equation}
Then, we calculate the derivative of $\alpha^t$ with respect to the global loss function $F(W^{t+1})$:
\begin{equation}
\label{eq:gderi}
\begin{split}
\frac{\partial F(W^{t+1})}{\partial \alpha^t} &= \nabla F(W^{t+1}) \cdot \frac{\partial (W^{t} - \alpha^t \nabla F(W^{t}))}{\partial \alpha^t} \\
&=-\nabla F(W^{t+1})\cdot\nabla F(W^{t})
\end{split}
\end{equation}

However, we cannot get $\nabla F(W^{t+1})$ in $t$th round, so we approximate $\frac{\partial F(W^{t+1})}{\partial \alpha^t}$ by $\frac{\partial F(W^{t})}{\partial \alpha^{t-1}}$, and get the following update rule for $\alpha^t$:
\begin{equation}
\label{eq:alphaa}
\widetilde{\frac{\partial F(W^{t+1})}{\partial \alpha^t}}= \frac{\partial F(W^{t})}{\partial \alpha^{t-1}} = -\nabla F(W^{t})\cdot\nabla F(W^{t-1})
\end{equation}

Therefore, in order to minimize global loss function $F(W^{t+1})$, we can calculate $\alpha^t$ by hypergradient descent on $\alpha^{t-1}$:
\begin{equation}
\label{eq:alpha}
\begin{split}
\alpha^t &= \alpha^{t-1} - \widetilde{\frac{\partial F(W^{t+1})}{\partial \alpha^t}}\\
&= \alpha^{t-1} + \nabla F(W^{t})\cdot\nabla F(W^{t-1})
\end{split}
\end{equation}

%$\nabla F(W^{t})$ is the gradient computed on global model. 
However, in FL, we cannot directly compute the gradient $\nabla F(W^{t})$ on the server, but the global update $\Delta^t$. Therefore, we use $\Delta^t$ and $\Delta^{t-1}$ to approximate $\nabla F(W^{t})$ and $\nabla F(W^{t-1})$ in \ref{eq:alpha}. Then, the adjusting strategy of our global scheduler \textsc{FedHyper-G} in $t$th round is:
\begin{equation}
\label{eq:alphafl}
\alpha^t = \alpha^{t-1} + \Delta^t\cdot\Delta^{t-1}
\end{equation}

This strategy indicates that the new global learning rate in $t$th round should be the global learning rate in the last round $\alpha^{t-1}$ plus the product of the global model updates in $t$th and $t-1$th round. In this case, if $\Delta^t\cdot\Delta^{t-1}$ is positive, i.e., the global updates in the last two rounds have similar directions, the global learning rate will increase. On the contrary, if the number is negative, it means the two global updates have significantly different directions, so the global learning rate will decrease.

The gradient descent function of the global learning rate above cleverly aligns with our expectations of an ideal learning rate scheduler in Section \ref{avg_alr}. Here we recall our toy examples that use a quadratic function as the loss function. In Figure \ref{fig:G} (a), the model parameters in $t-1$th and $t$th rounds, i.e., $W^{t-1}$ and $W^{t}$, are far from the optimal point $W_{opt}$. So we need a larger learning rate to accelerate the training. 
According to the global learning rate scheduler defined by Equation \ref{eq:alpha}, here the hypergradient of $\alpha^t$, $\Delta^t\cdot\Delta^{t-1}$ is positive because the two global model updates have the same direction. Therefore, the $\alpha^t$ is larger than the $\alpha^{t-1}$ and the model can speed up approaching $W_{opt}$ with as we expected.

In Figure \ref{fig:G} (b), $W^{t-1}$ is already close to $W_{opt}$. The $t-1$th model update $\Delta^{t-1}\cdot\alpha^{t-1}$ is too large that the model parameter crosses the optimal point $W_{opt}$ to another side of it. So here we need a smaller learning rate to help the parameter approach $W^{opt}$. In this case, the hypergradient of $\alpha^t$, $\Delta^t\cdot\Delta^{t-1}$ is negative
because $\Delta^{t}$ has a different direction from $\Delta^{t-1}$. The $\alpha^t$ will be smaller than $\alpha^{t-1}$. $W^{t+1}$ can be updated by the more suitable smaller learning rate $\alpha^t$ and get closer to $W^{opt}$.

\begin{figure}[h]
%\framebox[4.0in]{$\;$}
\hspace{0.5cm}
\begin{minipage}[t]{2.0in}
\centering
\includegraphics[trim=0mm 0mm 0mm 0mm, clip,width=2.3in]{G1.png}
\centerline{\footnotesize (a) Far from Optimum}
\end{minipage}
\hspace{1.0cm}
\begin{minipage}[t]{2.0in}
\centering
\includegraphics[trim=0mm 0mm 0mm 0mm, clip,width=2.3in]{G2.png}
\centerline{\footnotesize (b) Close to Optimum}
\end{minipage}
\caption{Two situations in global learning rate optimization.}
\label{fig:G}
\end{figure} 

Based on the toy examples above, we can conclude that our global scheduler can adjust the global learning rate properly according to the needs. This is because we use the model updates of the last two epochs to compute the hypergradient, which can reveal the real-time training situations, i.e., the model parameter is far away or close to the optimal point.

In addition, to ensure convergence and prevent gradient exploration, we clip $\alpha^t$ by a preset bound value $\gamma_\alpha$ in each round:
\begin{equation}
\label{eq:gamma}
\alpha_t = \min \{ \max \{ \alpha_t, \frac{1}{\gamma_{\alpha}} \}, \gamma_{\alpha} \}
\end{equation}

\textbf{Server-side local scheduler: FedHyper-SL.} The server-side local scheduler adopts the same hypergradient as the global scheduler. It adjusts all the local learning rates from selected clients synchronously. The local learning rates are also clipped by a preset bound value $\gamma_\beta$:
\begin{equation}
\label{eq:sls}
\begin{split}
\beta_m^t &= \beta_m^{t-1} + \Delta^t\cdot\Delta^{t-1}, \forall {m} \in \{ 0,1, ..., M \} \\
\beta_m^t &= \min \{ \max \{ \beta_t, \frac{1}{\gamma_{\beta}} \}, \gamma_{\beta} \}
\end{split}
\end{equation}

The updated local learning rates $\beta_m^t$ are sent to clients \emph{after} $t$th round. They will be used by clients in the local updates in the $t+1$th round.

\subsection{Scheduler with $\beta$ Gradient Descent}\label{sub:lo}

The global and server-side local schedulers are efficient. However, some FL trainers might expect to use a more fine-grained scheduler to get more performance improvement. To make {\n} also universal for these users, we provide the client-side local scheduler, i.e., \textsc{FedHyper-CL} that adjusts the local learning rate on the clients. \textsc{FedHyper-CL} outperforms \textsc{FedHyper-G} and \textsc{FedHyper-SL} in convergence speed and accuracy because the clients perform more fine-grained adjustment in every local batch, while the server only performs it between communication rounds.

\textbf{Client-side Local scheduler: FedHyper-CL.} Here we define a local training epoch as training on one batch of data. Similar to Equation\ref{eq:alphafl}, local learning rate in $k$th local epoch on client $m$ can be updated by:
\begin{equation}
\label{eq:betafl}
\begin{split}
\beta_m^{t,k} &= \beta_m^{t,k-1} + g_m(W^{t,k})\cdot g_m(W^{t,k-1}) \\
\end{split}
\end{equation}

The $g_m(W^{t,k})$ and $g_m(W^{t,k-1})$ are the gradients computed on the adjacent mini-batches. This local learning rate update strategy tends to minimize local loss $F_m()$ on the local batches. However, this method may lead to high local learning rates for some clients with easy-to-train local data. If among them, there is local training that exhibits significant deviations from the global training task, it can hinder the convergence of the global model, especially in non-iid setting~\citep{wang2020tackling}.

To solve this problem, inspired by our global scheduler, we aim to introduce global model updates to restrict the local learning rate optimization. Specifically, we add another item $g_m(W^{t,k})\cdot\Delta^{t-1}$ to the local learning rate update, where $\Delta^{t-1}$ is the global model update in the last round:
\begin{equation}
\label{eq:local}
\beta_m^{t,k} =\beta_m^{t,k-1} + g_m(W^{t,k})\cdot g_m(W^{t,k-1}) \cdot (1 + \varepsilon\cdot\frac{g_m(W^{t,k})\cdot\Delta^{t-1}}{|g_m(W^{t,k})\cdot\Delta^{t-1}|})
\end{equation}

Similarly, $\nabla F_m^\xi(W^{t,k})\cdot\Delta^{t-1}$ is a positive number when $\nabla F_m^\xi(W^{t,k})$ and $\Delta^{t-1}$ have similar direction, otherwise it is negative. This item tends to increase $\beta_m^{t,k}$ when the local model update has a similar direction with the global model update and decrease it when they exhibit significant discrepancies. It can prevent some clients from obtaining excessively high learning rates that could potentially impact global convergence.

This learning rate update rule in \ref{eq:local} is more complicated than that in the global update rule. Here we define $X = g_m(W^{t,k})\cdot g_m(W^{t,k-1}); Y = g_m(W^{t,k})\cdot\Delta^{t-1}$. The local learning rate in the following four situations will:

\begin{enumerate}[label=(\roman*)]
\item $X>0; Y>0$ as in Figure\ref{fig:local} (i), increase;
\item $X<0; Y<0$ as in Figure\ref{fig:local} (ii), decrease;
\item $X>0; Y<0$ as in Figure\ref{fig:local} (iii), increase if $|X|>|Y|$, otherwise decrease;
\item $X<0; Y>0$ as in Figure\ref{fig:local} (iv), increase if $|X|<|Y|$, otherwise decrease.
\end{enumerate}

\begin{figure}[h]
\centering
%\begin{minipage}[t]{2.5in}
%\centering
%\includegraphics[trim=0mm 0mm 0mm 0mm,clip,width=2.4in]{toy.png}\\
%\centerline{\footnotesize}
%\end{minipage}
%\hspace{0cm}
\begin{minipage}[t]{1.3in}
\centering
\includegraphics[trim=0mm 0mm 0mm 0mm, clip,width=1.4in]{L1.png}\\
\centerline{\footnotesize (i)}
\end{minipage}
\hspace{0cm}
\begin{minipage}[t]{1.3in}
\centering
\includegraphics[trim=0mm 0mm 0mm 0mm, clip,width=1.4in]{L2.png}\\
\centerline{\footnotesize (ii)}
\end{minipage}
\hspace{0cm}
\begin{minipage}[t]{1.3in}
\centering
\includegraphics[trim=0mm 0mm 0mm 0mm, clip,width=1.4in]{L3.png}\\
\centerline{\footnotesize (iii)}
\end{minipage}
\hspace{0cm}
\begin{minipage}[t]{1.3in}
\centering
\includegraphics[trim=0mm 0mm 0mm 0mm, clip,width=1.4in]{L4.png}\\
\centerline{\footnotesize (iv)}
\end{minipage}
\caption{Four situations in adjusting local learning rate.}
\label{fig:local}
\end{figure}

This client-side local scheduler takes both the global and local training situations into account and adopts global model updates to guide the local learning rate optimization. It enables faster convergence of the local model while preventing excessive client uploads that adversely affect the global model convergence.

After addressing the global and local schedulers, we obtain the full {\n} algorithm and show the cooperation of \textsc{FedHyper-G} and \textsc{FedHyper-CL} in Algorithm \ref{alg:work}. Note that \textsc{FedHyper-SL} uses the same hypergradient with \textsc{FedHyper-G} so it is not applied in order to simplify the algorithm. 

\begin{algorithm}[tb]
\caption{Workflow of {\n}}
\label{alg:work}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithmic}[1] 
\REQUIRE Initial Global Model $W^0$, Number of Communication Rounds $T$, Number of Selected Clients each Round $M$, Initial Global Learning Rate $\alpha^0$, Initial Local Learning Rate each Round $\beta^0 =\beta^1 = \beta^0 = ... = \beta^{T-1}$, Local Epoch number $K$, Local batches $\xi$;
\ENSURE Trained Global Model $W^T$;
\FOR{$t$ in $0, 1, ..., T-1$}
\STATE Server send $W^t$ and $\beta^t$ to all selected clients.
\renewcommand{\algorithmicrequire}
{ \textbf{Clients: FedHyper-CL}}
\REQUIRE 
\STATE Compute global model update $\Delta^{t-1} = W^t - W^{t-1}$
\STATE $\beta_m^{t,0} = \beta^t$
\FOR{$k$ in $0, 1, ..., K-1$}
\STATE Compute $g_m(W^{t,k})$ on $W^{t, k}$ and $\xi$,
\STATE Update local learning rate: $\beta_m^{t,k} =\beta_m^{t,k-1} + g_m(W^{t,k})\cdot g_m(W^{t,k-1}) \cdot (1 + \varepsilon\cdot\frac{g_m(W^{t,k})\cdot\Delta^{t-1}}{|g_m(W^{t,k})\cdot\Delta^{t-1}|})$
\STATE Clip: $\beta_m^{t,k} = \min \{ \max \{ \beta_m^{t,k}, \frac{1}{\gamma_{\beta}} \}, 
\gamma_{\beta} \}$
\STATE Local model update: $W_m^{k+1} = W_m^{k} - \beta_m^{t,k} \cdot g_m(W^{t,k})$
\ENDFOR
\STATE Send $\Delta_m^t = W_m^{t, K} - W^t$ to server.
\renewcommand{\algorithmicrequire}{\textbf{Server: FedHyper-G}}
\REQUIRE
\STATE Compute global model update: $\Delta^t = \Sigma P_m \Delta_m^t$
\STATE Update global learning rate: $\alpha^t = \alpha^{t-1} + \Delta^t\cdot\Delta^{t-1}$
\STATE Clip: $\alpha_t = \min \{ \max \{ \alpha_t, \frac{1}{\gamma_{\alpha}} \}, \gamma_{\alpha} \}$
\STATE Update global model: $W^{t+1} = W^t - \alpha^t \cdot \Delta^t$
\ENDFOR
\end{algorithmic} 
\end{algorithm}

